VSRD: Instance-Aware Volumetric Silhouette Rendering for Weakly Supervised 3D Object Detection

Monocular 3D object detection poses a significant challenge in 3D scene understanding due to its inherently ill-posed nature in monocular depth estimation. Existing methods heavily rely on supervised learning using abundant 3D labels, typically obtained through expensive and labor-intensive annotation on LiDAR point clouds. To tackle this problem, we propose a novel weakly supervised 3D object detection framework named VSRD (Volumetric Silhouette Rendering for Detection) to train 3D object detectors without any 3D supervision but only weak 2D supervision. VSRD consists of multi-view 3D auto-labeling and subsequent training of monocular 3D object detectors using the pseudo labels generated in the auto-labeling stage. In the auto-labeling stage, we represent the surface of each instance as a signed distance field (SDF) and render its silhouette as an instance mask through our proposed instance-aware volumetric silhouette rendering. To directly optimize the 3D bounding boxes through rendering, we decompose the SDF of each instance into the SDF of a cuboid and the residual distance field (RDF) that represents the residual from the cuboid. This mechanism enables us to optimize the 3D bounding boxes in an end-to-end manner by comparing the rendered instance masks with the ground truth instance masks. The optimized 3D bounding boxes serve as effective training data for 3D object detection. We conduct extensive experiments on the KITTI-360 dataset, demonstrating that our method outperforms the existing weakly supervised 3D object detection methods. The code is available at https://github.com/skmhrk1209/VSRD.

==> additional_visualization_results/monocular_3d_object_detection/main.tex <==
\subsection{Monocular 3D Object Detection}
\label{sec:additional_visualization_results/monocular_3d_object_detection}

\input{additional_visualization_results/monocular_3d_object_detection/weakly_supervised_setting/main}
\input{additional_visualization_results/monocular_3d_object_detection/semi_supervised_setting/main}


==> additional_visualization_results/monocular_3d_object_detection/semi_supervised_setting/main.tex <==
\subsubsection{Semi-Supervised Setting}
\label{sec:additional_visualization_results/monocular_3d_object_detection/semi_supervised_setting}

We show additional visualization results of semi-supervised monocular 3D object detection in \cref{fig:additional_visualization_results/monocular_3d_object_detection/semi_supervised_setting/monodetr} and \cref{fig:additional_visualization_results/monocular_3d_object_detection/semi_supervised_setting/monoflex}, comparing our method with MonoDETR \cite{MonoDETR} and MonoFlex \cite{MonoFlex}, respectively. The detectors fine-tuned on a subset of the whole data demonstrate enhanced performance, surpassing those trained on the whole data from scratch.


==> additional_visualization_results/monocular_3d_object_detection/weakly_supervised_setting/main.tex <==
\subsubsection{Weakly Supervised Setting}
\label{sec:additional_visualization_results/monocular_3d_object_detection/weakly_supervised_setting}

Additional visualization results of weakly supervised monocular 3D object detection can be seen in \cref{fig:additional_visualization_results/monocular_3d_object_detection/weakly_supervised_setting}. Compared with WeakM3D \cite{WeakM3D} and Autolabels \cite{Autolabels}, our method demonstrates superior performance in both perspective and bird's eye views. WeakM3D struggles to estimate the orientations of laterally moving objects accurately because it assumes that most cars are forward-facing, resulting in suboptimal estimation for laterally moving objects. In contrast, our method leverages pseudo labels generated by the proposed auto-labeling for 3D supervision without fixed priors, leading to more accurate orientation estimation. Furthermore, for the comparison with Autolabels, which faces challenges in accurately estimating 3D bounding boxes, particularly in their vertical locations, our method demonstrates superior 
performance, affirming the high quality of our pseudo labels.


==> additional_visualization_results/multi_view_3d_auto_labeling/main.tex <==
\subsection{Multi-View 3D Auto-Labeling}
We show more visualization results of the 3D bounding boxes optimized by our proposed multi-view 3D auto-labeling. As shown in \cref{fig:additional_visualization_results/multi_view_3d_auto_labeling}, it is evident that our proposed multi-view 3D auto-labeling demonstrates proficiency in accurately reconstructing instance surfaces, even in the presence of occlusions. For instance, for the occluded pink vehicle showcased in the second column, despite the challenge of occlusion, our approach effectively renders the surface details and optimizes the 3D bounding box, which verifies the strength of our proposed instance-aware volumetric rendering when dealing with scenes with complex geometric relationships among instances, such as occlusions. 

